Constraining Dark Matter-Proton Scattering from Molecular Cloud Ionization

Optically dense clouds in the interstellar medium composed predominantly of molecular hydrogen, known as molecular clouds, are sensitive to energy injection in the form of photon absorption, cosmic-ray scattering, and dark matter (DM) scattering. The ionization rates in dense molecular clouds are heavily constrained by observations of abundances of various molecular tracers. Recent studies have set constraints on the DM-electron scattering cross section using measurements of ionization rates in dense molecular clouds. Here we calculate the analogous bounds on the DM-proton cross section using the molecular Migdal effect, recently adapted from the neutron scattering literature to the DM context. These bounds may be the strongest limits on a strongly-coupled DM subfraction, and represent the first application of the Migdal effect to astrophysical systems.

==> unused.tex <==
\begin{gather}
    P_{\rm{ion.}}(Q)=
    \begin{cases}
        0 &, Q < 10^5 \textrm{ eV}\\
        10^{5.32377}\left(\frac{Q}{\rm{eV}}\right)^{-1.06952} &, 10^5 \textrm{ eV}<Q<10^7\textrm{ eV}\\
        1 &, Q > 10^7 \textrm{ eV}
    \end{cases}.
    \label{eqn:Pion}
\end{gather}
\ref{eqn:Pion} shows that for low enough Q, no detectable transition is likely to occur, while for high enough Q, it is almost guaranteed to occur.
